S$^2$Contact: Graph-based Network for 3D Hand-Object Contact Estimation with Semi-Supervised Learning

Despite the recent efforts in accurate 3D annotations in hand and object datasets, there still exist gaps in 3D hand and object reconstructions. Existing works leverage contact maps to refine inaccurate hand-object pose estimations and generate grasps given object models. However, they require explicit 3D supervision which is seldom available and therefore, are limited to constrained settings, e.g., where thermal cameras observe residual heat left on manipulated objects. In this paper, we propose a novel semi-supervised framework that allows us to learn contact from monocular images. Specifically, we leverage visual and geometric consistency constraints in large-scale datasets for generating pseudo-labels in semi-supervised learning and propose an efficient graph-based network to infer contact. Our semi-supervised learning framework achieves a favourable improvement over the existing supervised learning methods trained on data with `limited' annotations. Notably, our proposed model is able to achieve superior results with less than half the network parameters and memory access cost when compared with the commonly-used PointNet-based approach. We show benefits from using a contact map that rules hand-object interactions to produce more accurate reconstructions. We further demonstrate that training with pseudo-labels can extend contact map estimations to out-of-domain objects and generalise better across multiple datasets.

==> Figure/vis_in_the_wild/item.tex <==
\begin{figure}[h]
\centering
% \vspace{+0.1cm}
\includegraphics[width=1\linewidth]{Figure/vis_in_the_wild/vis_in_the_wild.pdf}
% \vspace{-0.7cm}
\caption{
Qualitative results on \emph{EPIC-Kitchens}~\cite{Damen2018EPICKITCHENS} and \emph{100 Days of Hands}~\cite{Shan20}.
}
% \vspace{-0.4cm}
\label{fig:vis_in_the_wild}
\end{figure}

==> Table/runtime/item.tex <==
% Please add the following required packages to your document preamble:
\newcolumntype{C}{>{\centering\arraybackslash}X}
\begin{table}[h]
\begin{center}
% \vspace{-0.2cm}
\caption{Comparison on computational requirements of different networks.}
\label{table:runtime}
% \vspace{-0.2cm}
\resizebox{0.9\linewidth}{!}{%
\begin{tabularx}{\linewidth}{l | C | C | C }
\toprule
 & Baseline & DGCNN \cite{wang2019dynamic} & Ours \\ 
\midrule 
Parameters & {\footnotesize1,424,138} &{\footnotesize530,442} & {\footnotesize587,658} \\
GPU memory (GB) & {\footnotesize13.3} & {\footnotesize21.1} & {\footnotesize10.4} \\
\bottomrule
\end{tabularx}
}
% \vspace{-0.6cm}
\end{center}
\end{table}
